CAMA: Energy and Memory Efficient Automata Processing in Content-Addressable Memories

Accelerating finite automata processing is critical for advancing real-time analytic in pattern matching, data mining, bioinformatics, intrusion detection, and machine learning. Recent in-memory automata accelerators leveraging SRAMs and DRAMs have shown exciting improvements over conventional digital designs. However, the bit-vector representation of state transitions used by all SOTA designs is only optimal in processing worst-case completely random patterns, while a significant amount of memory and energy is wasted in running most real-world benchmarks. We present CAMA, a Content-Addressable Memory (CAM) enabled Automata accelerator for processing homogeneous non-deterministic finite automata (NFA). A radically different state representation scheme, along with co-designed novel circuits and data encoding schemes, greatly reduces energy, memory, and chip area for most realistic NFAs. CAMA is holistically optimized with the following major contributions: (1) a 16x256 8-transistor (8T) CAM array for state matching, replacing the 256x256 6T SRAM array or two 16x256 6T SRAM banks in SOTA designs; (2) a novel encoding scheme that enables content searching within 8T SRAMs and adapts to different applications; (3) a reconfigurable and scalable architecture that improves efficiency on all tested benchmarks, without losing support for any NFA that is compatible with SOTA designs; (4) an optimization framework that automates the choice of encoding schemes and maps a given NFA to the proposed hardware. Two versions of CAMA, one optimized for energy (CAMA-E) and the other for throughput (CAMA-T), are comprehensively evaluated in a 28nm CMOS process, and across 21 real-world and synthetic benchmarks. CAMA-E achieves 2.1x, 2.8x, and 2.04x lower energy than CA, 2-stride Impala, and eAP. CAMA-T shows 2.68x, 3.87x and 2.62x higher average compute density than 2-stride Impala, CA, and eAP.

==> guidelines.tex <==
\section{Introduction}

This document provides instructions for submitting papers to the 54th International Symposium on Microarchitecture~{\textregistered} (MICRO 2021).  In an effort to respect the efforts of reviewers and in the interest of fairness to all prospective authors, we request that all submissions to MICRO 2021 follow the formatting and submission rules detailed below. Submissions that violate these instructions may not be reviewed, at the discretion of the program chairs, in order to maintain a review process that is fair to all potential authors. This document is itself formatted using the MICRO 2021 submission format. The content of this document mirrors that of the submission instructions that appear on the conference website. All questions regarding paper formatting and submission should be directed to the program chairs.

\subsection{Format Highlights}
\begin{itemize}
\item Paper must be submitted in printable PDF format.
\item Text must be in a minimum 10pt font, see Table~\ref{table:formatting}.
\item Papers must be at most 11 pages, not including references.
\item No page limit for references.
\item Each reference must specify {\em all} authors (no {\em et al.}).
\item Authors of {\em all} accepted papers will be required to give a
lightning presentation (about 90s) in addition to the regular
conference talk.
\end{itemize}

\subsection{Paper Evaluation Objectives} 
The committee will make every effort to judge each submitted paper on its own merits. There will be no target acceptance rate. We expect to accept a wide range of papers with appropriate expectations for evaluation---while papers that build on significant past work with strong evaluations are valuable, papers that open new areas with less rigorous evaluation are equally welcome and especially encouraged.

\section{Paper Preparation Instructions}

\subsection{Paper Formatting}

Papers must be submitted in printable PDF format and should contain a {\em maximum of 11 pages} of single-spaced two-column text, {\bf not including references}.  You may include any number of pages for references, but see below for more instructions.  If you are using \LaTeX~\cite{lamport94} to typeset your paper, then we suggest that you use the template here: \href{https://www.microarch.org/micro54/submit/micro54-latex-template.zip}{\LaTeX~Template}. This document was prepared with that template.  If you use a different software package to typeset your paper, then please adhere to the guidelines given in Table~\ref{table:formatting}. 

\begin{scriptsize}
\begin{table}[h!]
  \centering
  \begin{tabular}{|l|l|}
    \hline
    \textbf{Field} & \textbf{Value}\\
    \hline
    \hline
    File format & PDF \\
    \hline
    Page limit & 11 pages, {\bf not including}\\
               & {\bf references}\\
    \hline
    Paper size & US Letter 8.5in $\times$ 11in\\
    \hline
    Top margin & 1in\\
    \hline
    Bottom margin & 1in\\
    \hline
    Left margin & 0.75in\\
    \hline
    Right margin & 0.75in\\
    \hline
    Body & 2-column, single-spaced\\
    \hline
    Space between columns & 0.25in\\
    \hline
    Line spacing (leading) & 11pt \\
    \hline
    Body font & 10pt, Times\\
    \hline
    Abstract font & 10pt, Times\\
    \hline
    Section heading font & 12pt, bold\\
    \hline
    Subsection heading font & 10pt, bold\\
    \hline
    Caption font & 9pt (minimum), bold\\
    \hline
    References & 8pt, no page limit, list \\
               & all authors' names\\
    \hline
  \end{tabular}
  \caption{Formatting guidelines for submission.}
  \label{table:formatting}
\end{table}
\end{scriptsize}

{\em Please ensure that you include page numbers with your submission}. This makes it easier for the reviewers to refer to different parts of your paper when they provide comments. Please ensure that your submission has a banner at the top of the title page, similar to this document, which contains the submission number and the notice of confidentiality.  If using the template, just replace XXX with your submission number.

\subsection{Content}

Reviewing will be {\em double blind} (no author list); therefore, please do not include any author names on any submitted documents except in the space provided on the submission form.  You must also ensure that the metadata included in the PDF does not give away the authors. If you are improving upon your prior work, refer to your prior work in the third person and include a full citation for the work in the bibliography.  For example, if you are building on {\em your own} prior work in the papers \cite{nicepaper1,nicepaper2,nicepaper3}, you would say something like: "While the authors of \cite{nicepaper1,nicepaper2,nicepaper3} did X, Y, and Z, this paper additionally does W, and is therefore much better."  Do NOT omit or anonymize references for blind review.  There is one exception to this for your own prior work that appeared in IEEE CAL, arXiv, workshops without archived proceedings, etc.\, as discussed later in this document.

\noindent\textbf{Figures and Tables:} Ensure that the figures and tables are legible.  Please also ensure that you refer to your figures in the main text.  Many reviewers print the papers in gray-scale. Therefore, if you use colors for your figures, ensure that the different colors are highly distinguishable in gray-scale.

\noindent\textbf{References:}  There is no length limit for references. {\em Each reference must explicitly list all authors of the paper.  Papers not meeting this requirement will be rejected.} Authors of NSF proposals should be familiar with this requirement. Knowing all authors of related work will help find the best reviewers. Since there is no length limit for the number of pages used for references, there is no need to save space here.

\section{Paper Submission Instructions}

\subsection{Guidelines for Determining Authorship}
IEEE guidelines dictate that authorship should be based on a {\em substantial intellectual contribution}. It is assumed that all authors have had a significant role in the creation of an article that bears their names. In particular, the authorship credit must be reserved only for individuals who have met each of the following conditions:

\begin{enumerate}
\item Made a significant intellectual contribution to the theoretical development, system or experimental design, prototype development, and/or the analysis and interpretation of data associated with the work contained in the article;

\item Contributed to drafting the article or reviewing and/or revising it for intellectual content; and

\item Approved the final version of the article as accepted for publication, including references.
\end{enumerate}

A detailed description of the IEEE authorship guidelines and responsibilities is available \href{https://www.ieee.org/publications_standards/publications/rights/Section821.html}{here}. Per these guidelines, it is not acceptable to award {\em honorary } authorship or {\em gift} authorship. Please keep these guidelines in mind while determining the author list of your paper.

\subsection{Declaring Authors}
Declare all the authors of the paper upfront. Addition/removal of authors once the paper is accepted will have to be approved by the program chairs, since it potentially undermines the goal of eliminating conflicts for reviewer assignment.

\subsection{Areas and Topics}
Authors should indicate these areas on the submission form as well as specific topics covered by the paper for optimal reviewer match. If you are unsure whether your paper falls within the scope of MICRO, please check with the program chairs -- MICRO is a broad, multidisciplinary conference and encourages new topics.

\subsection{Revision of Previously-Reviewed\\ Manuscript}
If the manuscript has been previously reviewed and rejected and is now being submitted to MICRO, the authors are expected to provide a letter explaining how the paper has been revised for this current submission. Papers that have previously been reviewed and rejected that do not include a revision letter may be rejected without review. Note that it is not a requirement that papers be revised before being submitted to MICRO, but we expect a revision letter nonetheless, even if it states that the paper has not been revised. 

We encourage you to keep this letter concise and append additional information, such as a version of the paper that highlights the differences or any other material of your choice. While {\bf this letter is required for submission (with a deadline that will be one week after the paper submission deadline)}, the authors have control about who and when this letter will be shared with, by specifying one of the following options:

\begin{enumerate}
\item Shared with all reviewers during the initial review process
\item Shared with reviewers who declare that they reviewed a prior version and explicitly request the revision information
\item Shared along with the rebuttal
\item Shared only with paper discussion leads in preparation for PC discussion
\item Not shared with any PC member 
\end{enumerate}

\subsection{Declaring Conflicts of Interest}
Authors must register all their conflicts for their paper submission. Conflicts are needed to ensure appropriate assignment of reviewers. {\bf If a paper is found to have an undeclared conflict that causes a problem OR if a paper is found to declare false conflicts in order to abuse or ``game'' the review system, the paper may be rejected without review.} We use the following conflict of interest guidelines for determining the conflict period for MICRO 2021.  Please declare a conflict of interest (COI) with the following people for any author of your paper:

\begin{enumerate}
\item Your Ph.D. advisor(s), post-doctoral advisor(s), Ph.D. students,
      and post-doctoral advisees, forever.
\item Family relations by blood or marriage, or their equivalent,
      forever (if they might be potential reviewers).
\item People with whom you have collaborated in the last FOUR years, including:
  \begin{itemize}
  \item co-authors of accepted/rejected/pending papers,
  \item co-PIs on accepted/rejected/pending grant proposals,
  \item funders (decision makers) of your research grants, and researchers
      whom you fund.
  \end{itemize}
\item People (including students) who shared your primary institution(s) in the
last FOUR years.
\item Ongoing collaboration that has not yet resulted in a paper or proposal submission. Justification may be queried.
\item Other relationships, such as close personal friendship, that you think might tend
to affect your judgment or be seen as doing so by a reasonable person familiar
with the relationship.
\end{enumerate}

We would also like to emphasize that the following scenarios do {\em not} constitute a conflict:
\begin{enumerate}
\item Authors of previously-published, closely related work on that basis alone.
\item ``Service'' collaborations such as co-authoring a report for a professional organization, serving on a program committee, or co-presenting tutorials.
\item Co-authoring a paper that is a compendium of various projects with no true collaboration among the projects.
\item People who work on topics similar to or related to those in your papers.
\item Collaborators on large funded projects where there is no close collaboration and no joint benefit in the paper being accepted.
\end{enumerate}

We hope to draw most reviewers from the program committee, but others
from the community may also write reviews. {\bf Please declare all your conflicts (not just restricted to the PC).} When in doubt, please contact the program chairs.

Please note that all paper submissions require all authors to electronically sign a statement confirming their best effort to accurately identify potential reviewers with a conflict of interest, and importantly also {\bf assuring that each author will make no explicit attempt to directly or indirectly influence any reviewer opinion or decision about the submitted paper}. Importantly, we do not consider technical discussion of a paper's content or any other sharing of content from the paper to violate the above policy. 


\subsection{Concurrent Submissions and Workshops}

By submitting a manuscript to MICRO 2021, the authors guarantee that the manuscript has not been previously published or accepted for publication in a substantially similar form in any conference, journal, or the archived proceedings of a workshop (e.g., in the ACM/IEEE digital library) -- see exceptions below. The authors also guarantee that no paper that contains significant overlap with the contributions of the submitted paper will be under review for any other conference or journal or an archived proceedings of a workshop during the MICRO 2021 review period. Violation of any of these conditions will lead to rejection.

The only exceptions to the above rules are for the authors' own papers in (1) workshops without archived proceedings such as in the ACM/IEEE digital library (or where the authors chose not to have their paper appear in the archived proceedings), or (2) venues such as IEEE CAL or arXiv where there is an explicit policy that such publication does not preclude longer conference submissions.  In all such cases, the submitted manuscript may ignore the above work to preserve author anonymity. This information must, however, be provided on the submission form -- the program chairs will make this information available to reviewers if it becomes necessary to ensure a fair review.  As always, if you are in doubt, it is best to contact the program chairs.


Finally, the ACM/IEEE Plagiarism Policy (\href{http://www.acm.org/publications/policies/plagiarism_policy}{here} and \href{https://www.ieee.org/publications_standards/publications/rights/plagiarism_FAQ.html}{here}) covers a range of ethical issues concerning the misrepresentation of other works or one's own work.


==> rebuttal.tex <==
\clearpage

\setcounter{section}{0}
\setcounter{figure}{0}
\setcounter{page}{1}

We thank the reviewers for the insightful comments. Our responses to the major questions are as follows. 

\textbf{Novelty vs. Prior Work (\#A, \#B, \#G)}:
Existing in-memory automata accelerators are all based on one-hot vector representation for state matching, which has constant cost for each state regardless of the transition symbols, leading to inefficient memory usage and high energy in most scenarios. 
Even though Impala made the first attempt to tackle this issue, by splitting 8-bit symbols to 4-bit symbols, so that 256-bit one-hot state matching SRAMs can be replaced by two 16$\times$256 ones. However, because SRAM peripherals occupy > 80\% of SRAM access energy, reading two 16$\times$256 SRAM banks is more energy consuming than reading a single 256$\times$256 bank and thus the efficiency of Impala is actually lower than CA.

%However, across 21 real-world and synthesized benchmarks~\cite{becchi_workload_2008,wadden_anmlzoo_2016}, it is found that only 3$\%$ of matching resources are utilized in 86$\%$ of the time on average. Thus, in most scenarios, the 256-bit vector representation for state matching is inefficient in memory usage, which further result in performance and energy penalties due to larger memory arrays. 



The starting point of CAMA is to avoid one-hot encoding for state matching and a natural choice is to directly match the actual symbols for each state using CAMs. For an alphabet with size $\mathscr{A}$, this scheme will require $log_2\mathscr{A}$ bits $\times$ the number of symbols for each state. But this na\"ive approach is advantageous when the symbol-set size is very small. 
To address this, we propose a set of optimizations. First, to reduce the number of CAM entries for each state, we compress multiple symbols into a single entry, thus requiring wildcard matching. But conventional 16T Ternary CAMs for wildcard matching is more than two times larger than 6T SRAM. So we propose a 8T CAM cell to replace 16T TCAM, enabled by a special data coding (\S 3.2). This coding scheme is flexible and gives us a large optimization space for any given NFA. Depending on the alphabet size and transitions, the coding length and the mapping from original symbols to the encoded data can be optimized with the proposed algorithms (\S 4). On the other hand, we optimize the switch network in a way similar to eAP, but with a simpler and more practical implementation (\S 3.2). In order to support applications with denser and larger symbol sets, the switch network can also be reconfigured between RCB and normal modes (\S 3.2). 

Quantitatively comparing SOTA designs, access energy of our CAM varies from 2.67pJ to 16.9pJ depending on the number of enabled columns, while the energy of local switch is almost the same in all designs. After coding optimization, CAMA only requires 12\% more states than the baseline. CAMA-E takes advantages of the selectively enabled columns to save energy. In worst benchmark (Fermi), the average access energy is only 7.8pJ. CAMA-T's energy stays at 16.9pJ, which is slightly lower than CA and eAP's 19.45pJ. 2-stride Impala requires 30.6pJ to access two 16x256 SRAMs. In terms of area, CAMA reduces state matching memory to 17x256, which is the smallest among all. Overall, CAMA achieves significantly higher area and energy efficiency.

\textbf{Input Encoding and Output Reporting Overheads (\#A, \#B, \#G)}:
The end-to-end execution of the accelerator requires input and output buffer, reporting logic, and input encoder in CAMA. The implementation of IB and OB are common across all designs and their costs are highly application dependent, so none of the prior designs include them in evaluations and comparisons. We design our 128-entry IB and 64-entry OB to keep a similar interrupt frequency between input and output. The reporting overhead has been studied on ANMLZoo, showing 10 out of 12 benchmarks have less than 0.5 reports per cycle. Thus its energy is negligible compared to the NFA computings. 
Encoding is unique to CAMA and is implemented by a 256x34 6T SRAM bank which is after the input buffer. It only consumes about 2.57pJ per access in 28nm. This energy only occupies 4.36\% of the smallest Bro217 benchmark, and on average occupies only 0.1\% of total energy. Our evaluations always include input encoding. 

\textbf{Choice of Benchmarks and Comparisons with SOTA (\#A, \#B, \#C, \#F, \#G)}:
We use ANMLZoo, rather than AutomataZoo, as our benchmark, because (1) the AP chip with up to 48k states only supports ANMLZoo; (2) simulating an automata accelerator on large benchmarks in AutomataZoo too time and memory consuming; and (3) all recent papers, even those on FPGAs, e.g. CA~\cite{subramaniyan_cache_2017}, Impala~\cite{sadredini_impala_2020}, AP~\cite{dlugosch_efficient_2014}, FlexAmata~\cite{sadredini_flexamata_2020}, and Grapefruit~\cite{rahimi_grapefruit_2020} all adopted ANMLZoo for evaluations. Thus, we use ANMLZoo and Regex benchmarks for fair comparisons with prior works.
Evaluation setups and comparisons with SOTA are updated in \S 5 and \S6.



%We used the Symbol Class Size to reflect on the effect of negation and did experiments on the effect of negation on state numbers. Results are presented in Table~\ref{table:symbol}. According to the experiment results, we decide to set a threshold of 2 where if Symbol Class Size is 2 times larger than Negation Symbol Class Size, we choose Negation Symbol Class Size to process our encoding (1 would increase Fermi's state to 61066 and 3 would increase Snort and D9's state to 74717 and 14244).



\textbf{Hardware Reconfigurability (\#A)}:
CAM arrays include a bit-level mask to turn off unused search bits for power savings. When the 17-row CAM is configured to receive codes more than 17 bits, two CAMs in one tile are combined (\S 3.2). 
Our switch network supports RCB and normal modes, by combining two switch networks, this is different from using state matching arrays as in eAP. 
%CAMA's RCB is implemented differently from that of eAP, because (1) it uses a diagnose width of 43 compared to eAP's 21, (2) it reconfigures by combining switch networks instead of using state matching arrays, (3) it requires only 2 bit-lines in each column, which is much easier to implement physically.


\textbf{Performance on Dense or Large Symbol Class and Different Alphabet Size (\#A, \#D)}: 
For small alphabets, our algorithm will use less encoding bits. For larger alphabets, theoretical sensitivity analysis is infeasible because our coding is application dependent. However, we can construct worst-case NFAs and show the upper bound of memory usage is 32 entries of 17 bits. This will make CAMA worse than prior designs. But this scenario is rare in practice, and even when it happens, not every state will be taking this much memory. (\textbf{\#A})  In the evaluated benchmarks, the worst case is RandomForest, which increases the state count by 2.28x. This happens because its average symbol class size is 51.55, which is larger than our compression capability and has to be stored in more state entries. However, the total memory bits of CAMA is still smaller than that of CA, and the energy of CAMA-E remains the smallest. Also, EntityResolution actually doesn't get worse. Table~\ref{table:coding} is revised for clarity. (\textbf{\#D})



\textbf{Process Scalability and System Reliability (\#D, \#F)}:
Except the 8T CAM, every logic and memory modules in CAMA is conventional digital circuits that are scalable to the latest process nodes. The reliability and correctness analysis and optimization of the proposed 8T CAM is very similar to that of normal 8T SRAM, which is well studied. We have performed extensive Monte Carlo based reliability analysis of our 8T CAM with at least 6-sigma yield (99.99966\%). Further, the proposed 8T CAM array has been taped out and verified in 65nm. Given these reasons, we don't believe there is any correctness or reliability issue with CAMA (\textbf{\#F}), and its technology scalability is as good as normal 8T SRAMs and will benefit from smaller process nodes in a way almost identical to SRAMs (\textbf{\#D}).
%Section XXX is revised.


\textbf{Miscellaneous}: We use TSMC memory compiler. (\textbf{\#C})

The power-gating is achieved in the CAM circuit level based on inputs, no extra control or compiling is needed.(\textbf{\#G})

\S 4.1, \S4.2 and Table~\ref{table:symbol} are revised to clarify our optimization for Symbol Classes with Negations  (\textbf{\#A})



==> table.tex <==
\begin{table}[h!]
\caption{28nm delay and frequecy for different designs}
  \centering
  \begin{adjustbox}{width=0.47\textwidth, center}
  \begin{tabular}{cccccc}
    \hline
   % \textbf{design} & \textbf{state match}&
%    \textbf{global switch}& \textbf{proposed RCB}
    %& \textbf{proposed global}& \textbf{proposed normal}\\
    
    \multirow{2}{*}{\textbf{design}} & {\textbf{state}} & {\textbf{local}} & {\textbf{global}} & {\textbf{max fre}} &  {\textbf{operated fre}} \\
 {} & \textbf{matching} & \textbf{switch} & \textbf{switch} & \textbf{} & \textbf{}\\
    \hline
    \hline
    CA &xxx&xxx&xxx&xxx&xxx \\
    \hline
    CAMA & XXX&XXX&XXX&XXX&XXX\\
    \hline
    Impala&xxx&xxx&xxx&xxx&xxx\\
    \hline
    
  \end{tabular}
  \end{adjustbox}
  \label{table:28nmdelay}
\end{table}


\begin{table}[h!]
\caption{65nm delay and frequecy for different designs}
  \centering
  \begin{adjustbox}{width=0.47\textwidth, center}
  \begin{tabular}{cccccc}
    \hline
   % \textbf{design} & \textbf{state match}&
%    \textbf{global switch}& \textbf{proposed RCB}
    %& \textbf{proposed global}& \textbf{proposed normal}\\
    
    \multirow{2}{*}{\textbf{design}} & {\textbf{state}} & {\textbf{local}} & {\textbf{global}} & {\textbf{max fre}} &  {\textbf{operated fre}} \\
 {} & \textbf{matching} & \textbf{switch} & \textbf{switch} & \textbf{} & \textbf{}\\
    \hline
    \hline
    CA &xxx&xxx&xxx&xxx&xxx \\
    \hline
    CAMA & XXX&XXX&XXX&XXX&XXX\\
    \hline
    Impala&xxx&xxx&xxx&xxx&xxx\\
    \hline
    
  \end{tabular}
  \end{adjustbox}
  \label{table:65nmdelay}
\end{table}





 



  
